Understanding and Mitigating the Bias in Sample Selection for Learning with Noisy Labels

Learning with noisy labels aims to ensure model generalization given a label-corrupted training set. The sample selection strategy achieves promising performance by selecting a label-reliable subset for model training. In this paper, we empirically reveal that existing sample selection methods suffer from both data and training bias that are represented as imbalanced selected sets and accumulation errors in practice, respectively. However, only the training bias was handled in previous studies. To address this limitation, we propose a noIse-Tolerant Expert Model (ITEM) for debiased learning in sample selection. Specifically, to mitigate the training bias, we design a robust network architecture that integrates with multiple experts. Compared with the prevailing double-branch network, our network exhibits better performance of selection and prediction by ensembling these experts while training with fewer parameters. Meanwhile, to mitigate the data bias, we propose a mixed sampling strategy based on two weight-based data samplers. By training on the mixture of two class-discriminative mini-batches, the model mitigates the effect of the imbalanced training set while avoiding sparse representations that are easily caused by sampling strategies. Extensive experiments and analyses demonstrate the effectiveness of ITEM. Our code is available at this url \href{https://github.com/1998v7/ITEM}{ITEM}.

==> 2_related.tex <==
% \begin{table*}[t]
% \centering
% \small
% \caption{\small We compare ITEM with various selection-based methods over four perspectives.}
% \vspace{-2mm}
% \label{tab:related_work}
% \scalebox{0.8}{
% \setlength{\tabcolsep}{2mm}{
% \begin{tabular}{c|cccc}
% \toprule[1pt]
% Methods                      & Network architecture   & Selection-criterion specific    & Training debias  & Data debias\\ \midrule
% Co-teaching \cite{han2018co}, CoDis \cite{xia2023combating}          & Double-branch   & Small-loss criterion            &  \ding{55}       &  \ding{55}\\
% JoCoR \cite{wei2020combating}, DivideMix \cite{li2020dividemix}, ProMix \cite{wang2022promix}                   & Double-branch   & Small-loss criterion            &  \ding{51}       &  \ding{55}\\
% SFT \cite{wei2022self}, Late Stopping \cite{yuan2023late}                  & Single-branch   & Fluctuation-based selection     &  \ding{51}       &  \ding{55} \\         \midrule
% ITEM {\small (ours)}                & Mixture-of-Experts  & Not specific                    &  \ding{51}       & \ding{51} \\
% \bottomrule[1pt]  
% \end{tabular}}
% }
% \vspace{-2mm}
% \end{table*}

\begin{figure*}[t]
\centering
\subfloat[\footnotesize A corrupted selection tendency]{
\begin{minipage}[b]{0.6\linewidth}
\includegraphics[width=\linewidth]{fig/dynamic.pdf}
\end{minipage}}
\hfil
\subfloat[\footnotesize Class-level F-score]{
\begin{minipage}[b]{0.3\linewidth}
\includegraphics[width=\linewidth]{fig/dynamic_3.pdf}
\end{minipage}}
\vspace{-2mm}
\caption{\small We train ResNet-18 on Sym. 60\% CIFAR-100 with small-loss \cite{han2018co} and fluctuation-based noise filtering \cite{wei2022self}. (\textbf{a}) Results on small-loss. \emph{Left}: the class distribution of three training stages. \emph{Right}: dynamic numbers of four representative categories. (\textbf{b}) Results on two selection criteria. Visualization of the class-level selection performance $\text{\sffamily F}_k$ in 100- and 200-th  epoch. The average F-score among all classes is reported.}
\label{fig:vis}
\vspace{-2mm}
\end{figure*}

\subsection{Sample Selection for Learning with Noisy Labels} 
There are two main research lines in sample selection to tackle the adverse effect of noisy labels.

\emph{1) Robust selection criteria}. Previous sample selection methods normally exploit the memorization effect of DNNs, i.e., DNNs first memorize training data with clean labels and then those with noisy labels \cite{han2018co,xia2020robust}. The small-loss criterion \cite{han2018co} is a typical method stemming from the memorization effect, which splits the noisy training set via a loss threshold. The samples with small losses are regarded as clean samples. Some modified criteria based on the small-loss criterion were proposed in later works. For example, DivideMix \cite{li2020dividemix} leveraged a Gaussian Mixture Model to fit the loss distribution among all training data, which avoids manually setting a loss threshold.
% Similarly, Arazo \emph{et al.} \cite{arazo2019unsupervised} proposed a Beta Mixture Model to fit the loss distribution. 
In addition to the family of small loss criterion, some methods motivated by prediction fluctuation are designed. These methods observe that the model tends to give inconsistent prediction results for noisy samples and thus filter noisy labels by identifying high-frequency fluctuation samples. For example, some studies \cite{xia2022sample,zhou2020robust} introduce the uncertainty of loss to identify noisy labels. 


\emph{2) Robust network architecture}. Easily works based on constructing the noise transition matrix always resort to an additional adaptation layer at the top of the softmax layer \cite{goldberger2016training,jindal2016learning} or design a new dedicated architecture \cite{han2018masking,yao2018deep}. For example, the dropout model \cite{srivastava2014dropout} designs a dropout layer as regularization, whose output is normalized by the softmax function to avoid overfitting. Recently, a family of double-branch networks has been proposed, which integrates two networks with the same architecture and selects clean samples for another network. A majority of sample selection methods \cite{han2018co,yu2019does,wei2020combating,li2020dividemix} belong to this family. 
% Besides, better performance would be achieved when ensembling prediction results from two networks. Nevertheless, a recent work \cite{wei2023fine} combines the classifier model with a stochastic model, which aims for robust data transformation. 



% \emph{3) Robust training procedures}. Overall, current methods in sample selection always resort to a self-training manner, i.e., there is an iterative process between clean label selection and model training. However, the incorrect selection would degrade the subsequent model learning, which further enhances the biased selection in return.
% Recently, some robust training manners were proposed. Concretely, \cite{zhou2020robust} designed a framework based on curriculum learning \cite{bengio2009curriculum}, which starts with learning from clean data and then gradually moves to learn noisy-labeled data with pseudo labels. There are also some works \cite{mots2023deep,younesian2021qactor,zhang2015active} utilizing active learning \cite{settles2009active}. For example, Younesia \emph{et al.} \cite{younesian2021qactor} assumed there is an oracle who knows the ground truth for noisy labels. Its framework follows the paradigm of active learning that gradually modifies the label of noisy samples while holding a minimum number of Oracle queries.


% \textbf{Relations and difference.} 
% As shown in Table \ref{tab:related_work}, we compare our proposal ITEM with previous selection-based methods on four dimensions, which highlight the advantages of ITEM in the following aspects: 
% \begin{itemize}
% \setlength\itemsep{0mm}
%     \item \textit{Flexibility of the network structure}. To our knowledge, we are the first to apply a mixture-of-experts (MoE) structure to LNL. Despite the core idea of MoE and double-branch structure being similar (\textit{i.e.}, ensembling prediction results and the selection result over different views), MoE exhibits more flexibility. Expanding the number of experts is simple and only increases slight parameter counts (0.01 million per expert). By contrast, 
%     the double-branch structure is hardly extended to a three- or four-branch structure since the number of parameters. 
    
%     \item \textit{Expansibility of the framework}. Compared with previous selection-based methods, our proposal is agnostic to the selection criteria, which can be easily integrated with different selection criteria and improves their performance.
%     \item \textit{Debias learning}. Previous mainly focus on the accumulation error, a training bias. In this paper, we empirically show the existence of data bias (\textit{i.e.}, the imbalanced dataset selected by current selection criteria) and design an expert-based sampling strategy, which mitigates this bias by adjusting selection probabilities and increasing the visibility of underrepresented classes.
% \end{itemize}



% % \vspace{1mm}
% \subsection{Long-Tailed Classification} Current long-tailed classification methods can be roughly categorized into two strategies: 1) customize the data sampler to modify sampling frequency for different classes (including over-sampling the tail-class samples and under-sampling the head-class samples) \cite{buda2018systematic,byrd2019effect,he2009learning}, and 2) generate class-wise weights of training losses for improving the importance of tailed classes in terms of empirical risk minimization \cite{akbani2004applying,japkowicz2002class,liu2006influence,margineantu2000does}. 
% For example, Menon \emph{et al.} \cite{menon2020long} proposed a logit adjustment strategy based on label frequencies, encouraging a large relative margin between logits of rare versus dominant labels.

% Besides, real-world scenarios contain both noisy labels and imbalanced class distribution, where imbalanced distribution makes mitigating the negative impact of noise more difficult \cite{xia2021sample}. Many researchers currently focus on learning from imbalanced noisy datasets \cite{xia2023combating, zhang2023noisy, jiang2022delving, huang2022uncertainty, xia2021sample}. For example, CoDis \cite{xia2023combating} proposed to measure the discrepancy between two networks via the Jensen-Shannon (JS) divergence. CurveNet \cite{jiang2022delving} designed a meta-net to learn from loss curves and assign varying weights to different training samples.

% However, both strategies result in underfitting in the representation of head classes, \textit{i.e.}, the model eventually learns sparse feature representations for head classes \cite{cao2019learning,yang2020rethinking}. To overcome this issue, some studies \cite{liu2019large,wang2017learning} leverage the knowledge underlying head classes to promote the learning of tail classes. Cui \emph{et al.} \cite{cui2019class} designs a re-balance loss by computing the number of instances from each class and assigning different importance weights. Tang \emph{et al.} \cite{tang2020long} leverages causal learning and disentangles feature learning via backdoor adjustment.


\subsection{Mixture-of-Experts} Mixture-of-Experts (MoE), which belongs to a combination method, has great potential to improve performance in machine learning \cite{kotsiantis2006machine}. Earlier works on MoE mainly focus on dividing the problem space between different experts. Concretely, combining classifiers exhibits promising performance in classification tasks \cite{lorena2008review,rokach2010ensemble}, especially for the problem that involves a limited number of patterns, high-dimensional feature sets, and highly overlapped classes \cite{tran2011bspnn,kotsiantis2011incremental}. Nowadays, MoE has been applied to several fields, such as long-tailed classification \cite{wang2020long,xiang2020learning} and nature languages processing (NLP) \cite{zuo2021taming,zhou2022mixture}. 







% \begin{figure*}[ht]
% \centering
%     \begin{minipage}{0.64\linewidth}
%         \includegraphics[width=\linewidth]{fig/dynamic.pdf} \\
%         \subcaption{A corrupted selection tendency}
%         \label{fig:tendency}
%     \end{minipage} \hfil
%     \begin{minipage}{0.327\linewidth}
%         \includegraphics[width=\linewidth]{fig/dynamic_3.pdf} \\
%         \subcaption{Class-level F-score}
%         \label{fig:selection_bias}
%     \end{minipage}
%     % \vspace{-2mm}
% \caption{\small We train ResNet-18 on Sym. 60\% CIFAR-100 with small-loss \cite{han2018co} and fluctuation-based noise filtering \cite{wei2022self}. (\textbf{a}) Results on small-loss. \emph{Left}: the class distribution of three training stages. \emph{Right}: dynamic numbers of four representative categories. (\textbf{b}) Results on two selection criteria. Visualization of the class-level selection performance $\text{\sffamily F}_k$ in 100- and 200-th  epoch. The average F-score among all classes is reported.}
% \vspace{-3mm}
% \label{fig:vis}
% \end{figure*}

% \begin{figure}
% 	\centering
% 	\subcaptionbox{subtitle1\label{fig: resulta}}
% 	{\includegraphics[width=0.64\linewidth]{fig/dynamic.pdf}}
% 	\subcaptionbox{subtitle2\label{fig: resultb}}
% 	{\includegraphics[width=0.327\linewidth]{fig/dynamic_3.pdf}}
% 	\caption{figure's caption}\label{fig: result}
% \end{figure}





